Personalized Anomaly Detection in PPG Data using Representation Learning and Biometric Identification

Photoplethysmography (PPG) signals, typically acquired from wearable devices, hold significant potential for continuous fitness-health monitoring. In particular, heart conditions that manifest in rare and subtle deviating heart patterns may be interesting. However, robust and reliable anomaly detection within these data remains a challenge due to the scarcity of labeled data and high inter-subject variability. This paper introduces a two-stage framework leveraging representation learning and personalization to improve anomaly detection performance in PPG data. The proposed framework first employs representation learning to transform the original PPG signals into a more discriminative and compact representation. We then apply three different unsupervised anomaly detection methods for movement detection and biometric identification. We validate our approach using two different datasets in both generalized and personalized scenarios. The results show that representation learning significantly improves anomaly detection performance while reducing the high inter-subject variability. Personalized models further enhance anomaly detection performance, underscoring the role of personalization in PPG-based fitness-health monitoring systems. The results from biometric identification show that it's easier to distinguish a new user from one intended authorized user than from a group of users. Overall, this study provides evidence of the effectiveness of representation learning and personalization for anomaly detection in PPG data.

==> Figures/Fig4.tex <==

\begin{figure}[ht]
\vspace*{-0.3cm}
\centering

\includegraphics[width=10cm, height=6cm]{Representation_Results_Step1.pdf}

\caption{Mean Performance of Representation Learning Classification task(first step of the proposed framework) across all test subjects. The mean performance of each test subject (across five trained models) is depicted by the black bullet marker. Note that the standard deviation from the mean AUC of each test subject turned out to be too low, showing the stability and robustness of the model.}

\label{Figure4}
\end{figure}

==> Tables/Table1_AD.tex <==
% This table shows the results for Movement Detection for Both Detasets when the subject is sitting and Walking.

\begin{table}[h!]
\centering
\caption{Mean Test AUC performance of Movement Detection in the Generalized Scenario}
\label{Table1_AD}

\begin{tabular}{p{5cm}P{3.5cm}P{3.5cm}}
\toprule
\multirow{2}{*}{Anomaly Detection Methods} & \multicolumn{2}{c}{\textbf{Test AUC Performance}} \\ \cmidrule{2-3}
                                & \textbf{PTT-PPG Dataset} & \textbf{Dalia Dataset} \\ \midrule

MVN                       & $0.40 \pm 0.39$      & $0.78 \pm 0.15$        \\
RL-MVN                   & \textbf{0.91 $\pm$ 0.11} &   \textbf{0.87 $\pm$ 0.15}        \\[2mm]

IF                       & $0.28 \pm 0.35$      & $0.56 \pm 0.14$        \\
RL-IF                  & \textbf{0.90 $\pm$ 0.12} &   \textbf{0.86 $\pm$ 0.14}        \\[2mm]

PCA                      & $0.69 \pm 0.34$      & $0.77 \pm 0.19$        \\
RL-PCA                   & \textbf{0.90 $\pm$ 0.11} &   \textbf{0.86 $\pm$ 0.08}        \\[2mm]

\bottomrule
\end{tabular}
\end{table}







==> Tables/Table2_AD.tex <==
% This table shows the results for Movement Detection for Both Detasets when the subject is sitting and Walking. Personalized Version

\begin{table}[ht!]
\centering
\caption{Mean Test AUC performance of Movement Detection in the Personalized Scenario}
\label{Table2_AD}

\begin{tabular}{p{5cm}P{3.5cm}P{3.5cm}}
\toprule
\multirow{2}{*}{Anomaly Detection Methods} & \multicolumn{2}{c}{\textbf{Test AUC Performance}} \\ \cmidrule{2-3}
                                & \textbf{PTT-PPG Dataset} & \textbf{Dalia Dataset} \\ \midrule

MVN                       & $0.74 \pm 0.29$      & $0.93 \pm 0.08$        \\
RL-MVN                   & \textbf{0.98 $\pm$ 0.04} &   \textbf{0.94 $\pm$ 0.04}        \\[2mm]

IF                       & $0.37 \pm 0.31$      & $0.87 \pm 0.15$        \\
RL-IF                  & \textbf{0.96 $\pm$ 0.06} &   \textbf{0.93 $\pm$ 0.05}        \\[2mm]

PCA                      & $0.84 \pm 0.22$      & $0.94 \pm 0.07$        \\
RL-PCA                   & \textbf{0.95 $\pm$ 0.06} &   \textbf{0.92 $\pm$ 0.04}        \\[2mm]

\bottomrule
\end{tabular}
\end{table}

==> Tables/Table3_BI.tex <==

% Table 1

\begin{table}[h]
\centering
\caption{Mean Test AUC performance of Biometric Identification in a General Scenario (Group of people Normal) and one individual anomaly while performing two different activities}
\label{Table3_BI}

\begin{tabular}{p{3.5cm}P{3cm}P{3cm}P{3cm}P{3cm}} 
\toprule
\multirow{3}{3cm}{Anomaly Detectors} & \multicolumn{4}{c}{\textbf{Test AUC Performance}} \\ \cline{2-5}
                                & \multicolumn{2}{c}{\textbf{PTT-PPG Dataset}} & \multicolumn{2}{c}{\textbf{Dalia Dataset}} \\ \cmidrule{2-3} \cmidrule{4-5}
                                & \textbf{Sitting} & \textbf{Walking} & \textbf{Sitting} & \textbf{Walking} \\ \midrule

MVN        & $0.40 \pm 0.26$      & $0.38 \pm 0.22$    & $0.43 \pm 0.26$   & $0.41 \pm 0.28$    \\
RL-MVN    & \textbf{0.60 $\pm$ 0.23} &   \textbf{0.62 $\pm$ 0.15} & \textbf{0.54 $\pm$ 0.16} & \textbf{0.55 $\pm$ 0.12} \\[2mm]

IF       & $0.45 \pm 0.36$      & $0.43 \pm 0.34$    & $0.45 \pm 0.29$   & $0.40 \pm 0.29$    \\
RL-IF    & \textbf{0.60 $\pm$ 0.25} &   \textbf{0.66 $\pm$ 0.15} & \textbf{0.52 $\pm$ 0.16} & \textbf{0.54 $\pm$ 0.12} \\[2mm]

PCA      & $0.43 \pm 0.29$      & $0.40 \pm 0.29$    & $0.43 \pm 0.25$   & $0.41 \pm 0.29$    \\
RL-PCA   & \textbf{0.59 $\pm$ 0.20} &   \textbf{0.61 $\pm$ 0.14} & \textbf{0.53 $\pm$ 0.11} & \textbf{0.56 $\pm$ 0.11} \\[2mm]

\bottomrule
\end{tabular}
\end{table}

==> Tables/Table4_BI.tex <==


% Table 1

\begin{table}[h]
\centering
\caption{Mean Test AUC performance of Biometric Identification in a Person (anomaly) and one Person (normal) Scenario while performing two different activities}
\label{Table4_BI}

\begin{tabular}{p{3.5cm}P{3cm}P{3cm}P{3cm}P{3cm}} 
\toprule
\multirow{3}{3cm}{Anomaly Detectors} & \multicolumn{4}{c}{\textbf{Test AUC Performance}} \\ \cline{2-5}
                                & \multicolumn{2}{c}{\textbf{PTT-PPG Dataset}} & \multicolumn{2}{c}{\textbf{Dalia Dataset}} \\ \cmidrule{2-3} \cmidrule{4-5}
                                & \textbf{Sitting} & \textbf{Walking} & \textbf{Sitting} & \textbf{Walking} \\ \midrule

MVN        & $0.76 \pm 0.22$      & $0.63 \pm 0.28$    & $0.56 \pm 0.20$   & $0.55 \pm 0.23$    \\
RL-MVN    & \textbf{0.86 $\pm$ 0.08} &   \textbf{0.78 $\pm$ 0.09} & \textbf{0.74 $\pm$ 0.09} & \textbf{0.66 $\pm$ 0.11} \\[2mm]

IF       & $0.58 \pm 0.29$      & $0.52 \pm 0.28$    & $0.56 \pm 0.24$   & $0.50 \pm 0.25$    \\
RL-IF    & \textbf{0.86 $\pm$ 0.09} &   \textbf{0.81 $\pm$ 0.07} & \textbf{0.76 $\pm$ 0.09} & \textbf{0.68 $\pm$ 0.07} \\[2mm]

PCA      & $0.69 \pm 0.23$      & $0.64 \pm 0.28$    & $0.56 \pm 0.22$   & $0.56 \pm 0.25$    \\
RL-PCA   & \textbf{0.80 $\pm$ 0.11} &   \textbf{0.72 $\pm$ 0.10} & \textbf{0.70 $\pm$ 0.11} & \textbf{0.62 $\pm$ 0.08} \\[2mm]

\bottomrule
\end{tabular}
\end{table}

